Signed graph embedding: when everybody can sit closer to friends than enemies

Signed graphs are graphs with signed edges. They are commonly used to represent positive and negative relationships in social networks. While balance theory and clusterizable graphs deal with signed graphs to represent social interactions, recent empirical studies have proved that they fail to reflect some current practices in real social networks. In this paper we address the issue of drawing signed graphs and capturing such social interactions. We relax the previous assumptions to define a drawing as a model in which every vertex has to be placed closer to its neighbors connected via a positive edge than its neighbors connected via a negative edge in the resulting space. Based on this definition, we address the problem of deciding whether a given signed graph has a drawing in a given $\ell$-dimensional Euclidean space. We present forbidden patterns for signed graphs that admit the introduced definition of drawing in the Euclidean plane and line. We then focus on the $1$-dimensional case, where we provide a polynomial time algorithm that decides if a given complete signed graph has a drawing, and constructs it when applicable.

==> abstract.tex <==
  \emph{Signed graphs} are graphs with signed edges. They are commonly
  used to represent positive and negative relationships in social
  networks, e.g., friend/enemy or like/dislike.
  Community detection in social networks represents an active area of
  research, mostly dealing with unsigned graphs. While balance theory
  and clusterizable graphs deal with signed graphs, recent empirical
  studies have demonstrated that they fail to reflect some current
  practices in real social networks.
% Balance theory and clusterizable graphs fail to capture all social
  relations.  In this paper we address the issue of drawing signed
  graphs and capture such social interations. We relax the previous
  assumptions to define a drawing as a model in which every vertex has
  to be placed closer to its friends (neighbors connected through a
  positive edge) than its enemies (neighbors connected through a
  negative edge) in the resulting space.  Based on this definition, we
  address the problem of deciding whether a given signed graph has a
  drawing in a given $\ell$-dimensional Euclidean space. We then
  answer the question of finding the smallest dimension $\ell$ such
  that a given signed graph has a drawing in the $\ell$-dimensional
  Euclidean space if possible. More specifically, we provide an upper
  bound on the smallest dimension in which a given signed graph can be
  drawn. Then, we focus on the $1$-dimensional case, where we provide
  a polynomial time algorithm that decides if a given \emph{complete
  signed graph} has a drawing, and provides it when applicable. 
 Finally, we show how to use the the same algorithm to predict signed edges
  when the signed graph is not complete.


==> central-nodes.tex <==
\begin{definition}
Given a signed graph $G=(V,E^+\bigcupE^-)$, we say that a node $a_0 \in V$ us \emph{central} if and only if, for any $k$, there exists a set of $2k$ nodes $A=\{a_{-k}, a_{-k+1},\ldots,a_{-1},a_{1},a_2,\ldots,a_k\}$ such that nodes $a_0 \bigcup A$ induce the following subgraph of $G$:
$$
\widetilde{G} = (a_0 \bigcup A, E^+ =\{(a_i,a_{i+1}): -k \leq i \leq k-1\}) \bigcup E^- = \{(a_i,a_{i+k+1}): -k \leq i \leq -1\})
$$  
\end{definition}
\begin{definition}
Given a signed graph $G$ and a valid drawing $D(G)$, we say that node $a$ is placed in one extreme of $D(G)$ if either $p_a < p_i$ for all $i$ or $p_i< p_a$ for all $i$. 
\end{definition}

\begin{lemma}\label{lema.centralnode}
Given a signed graph $G$ with a central node $a_0$, then none valid drawing of $G$ makes $a_0$ an extreme node. 
\end{lemma}

\begin{proof}
The proof is by contradiction. Let us assume that $G$ has a central node $a_0$ and a valid drawing $D(G)$ that makes $a_0$ an extreme node. (W.l.o.g., we assume that $a_0$ is the \emph{left} node in $D(G)$, i.e., $p_{a_0} < p_i$ for all $i \in V$.) Since $a_0$ is a central node, then there exists such a set $A=\{a_{-k}, a_{-k+1},\ldots,a_{-1},a_{1},a_2,\ldots,a_k\}$ of nodes that makes $a_0$ a central node. Let us consider nodes $a_{-1},a_0, a_1, a_2, \ldots, a_{k-2}$ and their positions in $D(G)$, note that these nodes form a cycle without chords where every edge is positive but edge $(a_{-1},a_{k-2})$ which is negative. Now, $D(G)$ has two possibilities either it places the nodes such that $p_{a_{-1}} < p_{a_{k-2}}$ or vice versa $p_{a_{k-2}} < p_{a_{-1}}$. W.l.o.g, we assume the first case. Then, $D(G)$ has to place node $a_{-2}$ at the left of node $a_{k-3}$ ($p_{a_{-2}} < p_{a_{k-3}}$). Otherwise, if $p_{a_{k-3}} < p_{a_{-2}}$, we have two cases: 
\begin{itemize}
\item[Case $p_{a_{k-3}}<p_{a_{k-2}}$:]  In that case, since we are assuming that  $p_{a_{k-3}} < p_{a_{-2}}$, then we have $d(a_{k-3},a_{-2}) < d(a_{k-3},a_{k-2})$. Together with the fact that edge $(a_{k-3},a_{-2})$ is negative, and edge $(a_{k-3},a_{k-2})$ is positive, we obtain a contradiction. 
\item[Case $p_{a_{k-2}}<p_{a_{k-3}}$:] In this case,  since we are assuming that  $p_{a_{k-3}} < p_{a_{-2}}$ and the case says $p_{a_{k-2}}<p_{a_{k-3}}$, then we have $p_{a_{-1}}<p_{a_{k-3}} < p_{a_{-2}}$, which again produces a contradiction due to the fact that edge $(a_{-2},a_{-1})$ is positive and longer than edge $(a_{-2}, a_{k-3})$ which is negative.  
\end{itemize}
Repeating the same argument we have: $D(G)$ has to place node $a_{-3}$ at the left of node $a_{k-4}$, node $a_{-4}$ at the left of node $a_{k-5}$, and so on, until node $a_{-k+1}$ has to be placed at the left of node $a_0$, which is a contradiction with the fact that $a_0$ is the left node of $D(G)$.  
\end{proof}

\begin{corollary}
Let $G$ be a signed graph with a valid drawing, then $G$ has at least two nodes that aren't central. 
\end{corollary}
The proof follows directly from Lemma \ref{lemma.centralnode}. Indeed, assume that $G$ has one node that is not central, say it is placed in the left extreme of a valid drawing of $G$. Then, in the right extreme of that valid drawing there is central node, contradiction with Lemma \ref{lemma.centralnode}.

\begin{definition}
We define the signed graph named \emph{cycle type $k$} and denoted by $\mathcal{C}_k=(V,E^+\bigcup E^-)$ for a given value $1<k<n-1$. Let $V=\{0,1,2,\ldots,n-1\}$ be $\mathcal{C}_k$'s set of nodes and $E^+=\{(i,i+1)\mod n\}_{\forall i \in \{0,1,\ldots,n-1\} }$ $\mathcal{C}_k$'s set of positive edges. Now, for the given $1<k<n-1$, we define the set of negative edges in the following way: $E^-=\{(i,i+k)\mod n\}_{\forall i \in \{0,1,2,\ldots,n-1\}}$.
\end{definition}

==> counterexamples-resume.tex <==
In this section we present examples of signed graphs without valid
drawing in dimension $1$ and $2$.  Specifically, we present three
signed graphs, (resp. two), for which we prove they do not have
 a valid drawing in $\mathbb{R}$, (resp.  $\mathbb{R}^2$).
%Also, we explain, 
%from these examples and for a given dimension $\ell$, how to obtain a signed
%graph without valid drawing in $\mathbb{R}^\ell$. 
We conclude this section with the introduction    
of the concept of \emph{minimal signed graph without valid drawing}, and with a discussion about its consequences.

\paragraph{Signed graphs without valid drawing in the line}
%
Let us start presenting the counterexamples in increasing order with respect to the number of vertices. 
%
%

%\noindent
{\bf Positive square:} The first counterexample is a signed
graph composed of four vertices connected in a square of positive
edges, while the diagonals are assigned negative
signs. Fig. \ref{counterexampledim1}\textit{(a)} depicts the described
signed graph, let us refer to this signed graph as \emph{the positive square}.
%
%\begin{lemma}\label{lem:positivesquare}
%Let $G$ be the positive square signed graph, then $G$ has not a valid drawing in the Euclidean line $\mathbb{R}$.
%\end{lemma}
%\begin{proof} 
%Assume that there exists a valid drawing for the positive square
%in the line and let us achieve a contradiction starting from this valid drawing.
%Since vertices are placed in the line, let us number the vertices from left to right hand side. 
%Let us call vertex $p_1$ to the vertex that is placed most at the left in the line, the next vertex is called vertex $p_2$, then vertex $p_3$, 
%and the vertex placed most at the right is called vertex $p_4$. 
%Then there are two possibilities, either vertices $p_2$ and $p_3$ are connected 
%by a negative edge, or they are connected by a positive edge. 
%When vertices $p_2$ and $p_3$ are connected by a positive edge, then 
%vertices $p_1$ and $p_4$ are also connected by a positive edge, and vertices $p_1$ and $p_3$ are connected by a negative edge. 
%Hence, the contradiction comes from the fact that the positive edge that connects vertices $p_1$ and $p_4$ is longer than the 
%negative edge that connects vertices $p_1$ and $p_3$, both edges being adjacent to $p_1$. On the other hand, if vertices $p_2$ and $p_3$ are connected by a negative edge, 
%then vertices $p_1$ and $p_4$ are also connected by a negative edge, and vertices $p_1$ and $p_3$ are connected by a positive edge. 
%In that case, the contradiction comes from the fact that the negative edge that connects vertices $p_2$ and $p_3$ is shorter 
%than the positive edge that connects vertices $p_1$ and $p_3$, both edges being adjacent to $p_3$. Therefore, there is a contradiction, and we conclude that there 
%is not such a valid drawing of the positive square signed graph in $\mathbb{R}$.
%\end{proof} 
%

{\bf Positive star:} The second counterexample is also a signed graph composed of four vertices. In this case, 
there is a central vertex connected with positive edges to the other three vertices. While, the three other vertices are connected 
among them via a triangle of negative edges. Fig. \ref{counterexampledim1}\textit{(b)} shows the described signed graph. Let us call 
this second graph \emph{the positive star}. 
%\begin{lemma}\label{lem:positivestar}
%Let $G$ be the positive star signed graph, then $G$ has not a valid drawing in the Euclidean line $\mathbb{R}$.
%\end{lemma}
%\begin{proof}
%The proof is by contradiction. We assume that $G$ has a valid drawing in the line, and we call it $D(G)$. 
%Note that, by The Pigeon Hole Principle, in every drawing of the positive star in the line, 
%the central vertex, the one that is connected by 
%positive edges to the three other vertices, must have at least two vertices at one side, either its left or its right hand side. 
%In particular, that is true for $D(G)$. Without loss of generality, we assume that in $D(G)$ there are two vertices 
%placed at the right hand side of the central vertex. Let us call $p_1$ the central vertex, $p_2$ the first vertex at 
%the right hand side of the central vertex, and $p_3$ the second vertex from left to right placed at the right hand 
%side of the central vertex. Hence, the contradiction comes from the fact that vertices $p_1$ and $p_3$ are connected by a positive edge, 
%while vertices $p_2$ and $p_3$ are connected by a negative edge. Therefore, $p_3$ generates the contradiction because 
%the positive edge that connects vertices $p_1$ and $p_3$ is longer that the negative edge that connects $p_2$ and $p_3$. Then, 
%we conclude that the positive star has not a valid drawing in the line. 
%\end{proof}
%

{\bf Positive triangle:} The last counterexample is a signed graph with six vertices, three of them are clustered 
with positive edges in a central triangle. Each external vertex, those that are not
in the central triangle, is matched via a positive edge with one corner of the triangle, and connected via a negative edge with the 
other two corners of the triangle. Fig. \ref{counterexampledim1}\textit{(c)} shows precisely the described signed graph. Let us call 
this last graph \emph{the positive triangle}.

\begin{lemma}\label{lem:positivetriangle}  
Let $G$ be a signed graph. If $G$ is either the positive square or the positive star or the positive triangle, then $G$ has not a valid drawing in the Euclidean line $\mathbb{R}$.
\end{lemma}
%
\begin{figure}[t]
\begin{center}
\includegraphics[height=1in]{counterexampleline}
\caption{This figure shows signed graphs \textit{(a)} \emph{the positive square}, \textit{(b)} \emph{the positive star}, \textit{(c)} \emph{the positive triangle}. Dashed lines represent negative edges and continuous lines represent positive edges.}
\label{counterexampledim1}
\end{center}
\end{figure}
%
%\begin{proof}
%The proof is by contradiction. Let us start from $D(G)$ a valid drawing of $G$ in the line. 
%The first fact we point out says that in a valid drawing of $G$ the three vertices connected via a positive triangle 
%must be placed consecutively in the line, i.e., there can not be any external vertex placed among them. 
%The reason why it can not happen is the following: assume there is one external vertex placed in the 
%middle of the positive triangle, let us call it vertex $p_e$. Then, by The Pigeon Hole Principle, there are two 
%vertices of the triangle placed at one side of $p_e$ 
%and the reminder vertex is placed at the other side of the $p_e$, let us denote that vertex $p_b$. Necessarily, one vertex of the triangle, 
%among the two that are placed at the same side of $p_e$, is connected by a negative edge with $p_e$, let us denote that vertex $p_a$. 
%Also, $p_a$ is connected by a positive edge with $p_b$. 
%Hence, the contradiction comes from the fact that the positive edge that connects $p_a$ with $p_b$ is longer than the
%negative edge that connects $p_a$ with $p_e$, both edges being adjacent to $p_e$. Then, $D(G)$ places the three vertices of the triangle consecutively in the line. 
%
%Now, since we know that the three vertices of the positive triangle are placed consecutively in the line, and again by The Pigeon Hole Principle, there are at least 
%two external vertices placed at the same side of the positive triangle. 
%Without loss of generality, we assume that there are two external vertices placed at the left of the positive triangle. 
%Let us denote $p_l$ the leftest vertex being part of the positive triangle. Notice that $p_l$ is connected by a negative 
%edge with at least one of the external vertices at its left, let us call $p_a$ that vertex. Also, notice that $p_a$ is connected 
%by a positive edge with a vertex of the triangle that is at the right hand side of $p_l$, let us denote this vertex with $p_r$. Hence 
%the contradiction comes from the fact that the negative edge that connects vertices $p_a$ and $p_l$ is shorter than the positive 
%edge that connects vertices $p_a$ and $p_r$, both edges being adjacent to $p_a$. Therefore, we conclude that such a valid drawing $D(G)$ does not exist.       
%\end{proof}
\paragraph{Signed graphs without valid drawing in the plane}
%The Euclidean plane is a more complex structure than the Euclidean line. Therefore. 
%, the arguments used  to prove that a signed graph has not a valid drawing in the plane have to be more complex.  
In the plane we have found two signed graphs without valid drawing.
%
%
%
%\noindent

{\bf Negative triangle:} The \emph{negative triangle} is a graph of five vertices, three of them, forming a triangle, being connected
by negative edges. The other two vertices
 are connected by a negative edge. The other edges are positive.  
Fig. \ref{counterexampledim2}\textit{(a)} depicts the negative triangle. 
%\begin{lemma}\label{lem:signedhexagon} 
%Let $G$ be the negative triangle signed graph, then $G$ has not a valid drawing in the Euclidean plane $\mathbb{R}^2$.
%\end{lemma}
%\input{proofl4}
%

{\bf Negative cluster:} The \emph{negative cluster} is a signed graph with seven vertices. Six vertices out of the seven
are connected in a cluster of negative edges. The seventh vertex, called central vertex, is connected with positive edges 
with each of the six vertices in the cluster. Fig. \ref{counterexampledim2}\textit{(b)} depicts the negative cluster. 
\begin{lemma}\label{lem:negativecluster}
Let $G$ be a signed graph. If $G$ is either the negative triangle or the negative cluster, then $G$ has not a valid drawing in the Euclidean plane $\mathbb{R}^2$.
\end{lemma}
%%
%%
%
%
%%
%%
%\input{proofl5}
\paragraph{Minimal graphs without valid drawing} 
An interesting remark about graphs with valid drawing in a given dimension 
is the fact that the property of having a valid drawing in a given dimension 
is heritable through subgraphs.  This can be stated as follows. 
%\begin{remark}\label{rem:inclusion}
\emph{Let $G$ be a signed graph. Then, $G$ has no  valid drawing in $\mathbb{R}^\ell$ if and only if 
there exists a subgraph of $G$ that has no valid drawing in $\mathbb{R}^\ell$.} 
%\end{remark}
Pushing previous remark %\ref{rem:inclusion} 
to the extreme case when the only subgraph without valid drawing is the same graph, 
then we obtain the definition of \emph{minimal graph without valid drawing}. 
%
\begin{definition}\label{def:minimal}
Let $G$ be a signed graph without valid drawing in $\mathbb{R}^\ell$. We say that $G$ is \emph{minimal} 
%signed
%graph without valid drawing in $\mathbb{R}^\ell$ 
%if and only if 
when every proper subgraph of $G$ has a valid drawing in 
$\mathbb{R}^\ell$.  
\end{definition}
%AMK: again connfused with the meaning of proper...

At this point, and using Definition \ref{def:minimal}, we state a complementary problem to 
the one stated in Section \ref{sec:problem}.
%
%\begin{definition}\label{def:complementaryproblem}
Let us denote $\mathcal{M}^\ell$ the set of all minimal graphs without valid drawing in $\mathbb{R}^\ell$. 
The complementary problem consists in \emph{give a complete characterization} of $\mathcal{M}^\ell$.
%\end{definition}
The interest of this problem arises in the search of forbidden patterns in signed graphs such that they
have a valid drawing.
Since, the property of having a valid drawing is heritable
through subrgaphs. Then, a signed graph $G$ has not a valid drawing in $\mathbb{R}^\ell$ if and only if $G$ does not contain 
as subgraph any $G'$ in $\mathcal{M}^\ell$. Our contribution to the complementary problem follows.
%is the fact 
%that every signed graph described previously in this section gives a signed graph that is either in 
%$\mathcal{M}^1$ or in $\mathcal{M}^2$.
\begin{theorem}
Let $G_1$ be the positive square signed graph and $G_2$ be the positive star signed graph, then $\{G_1,G_2\}$ is a subset of $\mathcal{M}^1$.
\end{theorem}
%\input{prooft1}
\begin{theorem}
Let $F_1$ be the negative triangle signed graph and $F_2$ be the cluster signed graph, then $\{F_1,F_2\}$ is a subset of $\mathcal{M}^2$.
\end{theorem}
\begin{figure}[t]
\begin{center}
\includegraphics[height=1in]{counterexampleplane}
\caption{This figure shows two signed graphs \textit{(a)} \emph{the negative triangle} and \textit{(b)} \emph{the negative cluster}.
 Dashed lines represent negative edges and continuous lines represent positive edges.}
\label{counterexampledim2}
\end{center}
\end{figure}




==> generalcase.tex <==
In this section, we present two results related with the general case. 
Our first result says that if a signed graph has a valid drawing in 
$\mathbb{R}^\ell$, then also it has a valid drawing in $\mathbb{Q}^\ell$ and 
in $\mathbb{N}^\ell$. This result changes the geometric appeal of the problem. 
The fact that a signed graph has a valid drawing in a continuous space if 
and only if it has a valid drawing in a grid opens the possibility to use 
combinatorial ideas.   

In order to state the first result, note that the definition of drawing a graph 
in $\mathbb{R}^\ell$ can be straightforwardly restated for drawing a graph in $\mathbb{Q}^\ell$
and drawing a graph in $\mathbb{N}^\ell$. It is just required that the points that determine the position 
of the vertices are now in either $\mathbb{Q}^\ell$ or $\mathbb{N}^\ell$, respectively. 
Furthermore, also the definition of valid drawing can be restated for
$\mathbb{Q}^\ell$ or $\mathbb{N}^\ell$. Again, it is just required that the points in 
a valid drawing are now in either $\mathbb{Q}^\ell$ or $\mathbb{N}^\ell$, respectively. 
\begin{lemma}\label{lem:grid}
Given a signed graph $G$, the three statements that follow are equivalent. 
\begin{itemize}
\item $G$ has a valid drawing in $\mathbb{R}^\ell$
\item $G$ has a valid drawing in $\mathbb{Q}^\ell$
\item $G$ has a valid drawing in $\mathbb{N}^\ell$.
\end{itemize}
\end{lemma}
\begin{proof}
Using the inclusion of $\mathbb{N}^\ell$ in $\mathbb{Q}^\ell$, and also the inclusion of $\mathbb{Q}^\ell$ in $\mathbb{R}^\ell$, 
it is straightforward to conclude that a valid drawing in $\mathbb{N}^\ell$ implies a valid drawing in $\mathbb{Q}^\ell$, 
and also it implies a valid drawing in $\mathbb{R}^\ell$. Now, we have to prove the opposite direction of the equivalence. 
We start pointing out the fact that, because of the strict inequalities in Definition \ref{def:properdrawing}, 
given a signed graph $G$, the set of all valid drawings of $G$ in $\mathbb{R}^\ell$
is an open set in $\mathbb{R}^{n\ell}$.
Therefore, if that set is not empty,
it contains an element of $\mathbb{Q}^{n\ell}$. That comes from the fact that $\mathbb{Q}^{n\ell}$ is a dense set in $\mathbb{R}^{n\ell}$. 
Then, every open set in $\mathbb{R}^{n\ell}$ contains an element of $\mathbb{Q}^{n\ell}$.
(For further insights on mathematical analysis, we refer the reader to \cite{rudin-principles}.)
In other words, if $G$ has a valid drawing in $\mathbb{R}^\ell$, it has a valid drawing in $\mathbb{Q}^\ell$.

On the other hand, given that every inequality remains valid if it is multiplied by the same 
positive value at both sides of it. Then, we point out the fact that if every component of a valid 
drawing of $G$ is multiplied by the same positive value, the result is also a valid drawing of $G$. 
That is because, multiply for the same value every component of a valid drawing is seen in the inequalities that 
determine a valid drawing as a multiplication of every inequality for the same positive value at both sides of them.     

Therefore, given a valid drawing of $G$ in $\mathbb{Q}^\ell$, 
it is possible to obtain a valid drawing of $G$ in $\mathbb{N}^\ell$ by multiplying  
every element of the valid drawing in $\mathbb{Q}^\ell$ by the least common multiple 
among all of them. Therefore, the result is a valid drawing of $G$ that lies in $\mathbb{N}^\ell$. 
\end{proof}
%

%The second result that we show in this section is an upper bound on the dimension 
%in which a signed graph has a valid drawing. In other words, given a signed graph $G$, 
%the result gives a value $\ell(G)$ such that $G$ has a valid drawing in $\mathbb{R}^{\ell(G)}$. 
%Nevertheless, the bound provided here is not tight as we show with an example. 
%\begin{lemma}\label{lem:upperbound}
%Given a signed graph $G=(V,E^+\bigcup E^-)$, there exists $\ell(|V|,|E^-|)$ such that 
%$G$ has a valid drawing in $\mathbb{R}^{\ell(|V|,|E^-|)}$.
%\end{lemma}
%\begin{proof}
%...TO BE COMPLETED....
%\end{proof}

